Infrared Emission of Specific Polycyclic Aromatic Hydrocarbon Molecules: Indene

Polycyclic aromatic hydrocarbon (PAH) molecules have long been suggested to be present in the interstellar medium (ISM). Nevertheless, despite their expected ubiquity and sustained searching efforts, identifying specific interstellar PAH molecules from their infrared (IR) spectroscopy has so far been unsuccessful. However, due to its unprecedented sensitivity, the advent of the James Webb Space Telescope (JWST) may change this. Meanwhile, recent years have witnessed breakthroughs in detecting specific PAH molecules (e.g., indene, cyanoindene, and cyanonaphthalene) through their rotational lines in the radio frequencies. As JWST holds great promise for identifying specific PAH molecules in the ISM based on their vibrational spectra in the IR, in this work we model the vibrational excitation of indene, a molecule composed of a six-membered benzene ring fused with a five-membered cyclopentene ring, and calculate its IR emission spectra for a number of representative astrophysical regions. This will facilitate JWST to search for and identify indene in space through its vibrational bands and to quantitatively determine or place an upper limit on its abundance.

==> abstract.tex <==

Infrared Emission of Specific Polycyclic Aromatic Hydrocarbon Molecules: Indene


215 words

Polycyclic aromatic hydrocarbon (PAH) molecules have long been suggested to be present in the interstellar medium (ISM), owing to the close resemblance of their
characteristic infrared (IR) emission features to the so-called ``unidentified IR emission'' (UIE) bands at 3.3, 6.2, 7.7, 8.6, 11.3 and 12.7 micron that are ubiquitously seen in a wide variety of astrophysical regions. Nevertheless, despite their expected ubiquity and sustained searching efforts, identifying specific interstellar PAH molecules from their IR spectroscopy has so far been unsuccessful. However, due to its unprecedented sensitivity, the advent of the James Webb Space Telescope (JWST) may change this. Very recently, radio observations of the Taurus Molecular Cloud detected the rotational lines of indene (C9H8), a PAH molecule composed of a six-membered benzene ring fused with a five-membered cyclopentene ring and an essential building block of nonplanar PAHs. This represents the first definitive assignment of a specific, pure PAH molecule in space. As JWST holds great promise for identifying specific PAH molecules in the ISM, in this work we model the vibrational excitation of indene and calculate its IR emission spectra for a number of representative astrophysical regions.
This will facilitate JWST to search for and identify indene in space through its vibrational bands and to quantitatively determine or place an upper limit on its abundance.

KaijunLi

likaijun@stu.xmu.edu.cn

xjyang@xtu.edu.cn

fangt@xmu.edu.cn


Department of Astronomy, Xiamen University, Xiamen, Fujian 361005, China

Department of Physics and Astronomy, University of Missouri, Columbia, MO 65211, USA

Hunan Key Laboratory for Stellar and Interstellar Physics and School of Physics and Optoelectronics, Xiangtan University, Hunan 411105, China



Revised version: 169 words

Polycyclic aromatic hydrocarbon (PAH) molecules have long been suggested to be present in the interstellar medium (ISM). Nevertheless, despite their expected ubiquity
and sustained searching efforts, identifying specific interstellar PAH molecules from their infrared (IR) spectroscopy has so far been unsuccessful. However, due to its unprecedented sensitivity, the advent of the James Webb Space Telescope (JWST) may change this. Meanwhile, recent years have witnessed breakthroughs in detecting specific PAH molecules (e.g., indene, cyanoindene, and cyanonaphthalene) through their
rotational lines in the radio frequencies. As JWST holds great promise for identifying 
specific PAH molecules in the ISM based on their vibrational spectra in the IR, in this work we model the vibrational excitation of indene, a molecule composed of a six-membered benzene ring fused with a five-membered cyclopentene ring, and calculate its IR emission spectra for a number of representative astrophysical regions. This will facilitate JWST to search for and identify indene in space through its vibrational bands and to quantitatively determine or place an upper limit on its abundance.
